Benchmark Data and Evaluation Framework for Intent Discovery Around COVID-19 Vaccine Hesitancy

The COVID-19 pandemic has made a huge global impact and cost millions of lives. As COVID-19 vaccines were rolled out, they were quickly met with widespread hesitancy. To address the concerns of hesitant people, we launched VIRA, a public dialogue system aimed at addressing questions and concerns surrounding the COVID-19 vaccines. Here, we release VIRADialogs, a dataset of over 8k dialogues conducted by actual users with VIRA, providing a unique real-world conversational dataset. In light of rapid changes in users' intents, due to updates in guidelines or in response to new information, we highlight the important task of intent discovery in this use-case. We introduce a novel automatic evaluation framework for intent discovery, leveraging the existing intent classifier of VIRA. We use this framework to report baseline intent discovery results over VIRADialogs, that highlight the difficulty of this task.

==> intent_list.tex <==
\begin{table}
\small
\begin{center}
\begin{tabular}{ |p{7cm}|  }
\hline
intent\\ 
\hline
COVID-19 is not as dangerous as they say\\ 
\hline
Do I need to continue safety measures after getting the vaccine?\\ 
\hline
How long until I will be protected after taking the vaccine?\\ 
\hline
How many people already got the vaccine?\\ 
\hline
I am afraid the vaccine will change my DNA\\ 
\hline
I am concerned getting the vaccine because I have a pre-existing condition\\ 
\hline
I am concerned I will be a guinea pig\\ 
\hline
 I'm concerned the vaccine will make me sick.\\ 
\hline
I am not sure if I can trust the government\\ 
\hline
I am young and healthy so I don't think I should vaccinate\\ 
\hline
I distrust this vaccine\\ 
\hline
How much will I have to pay for the vaccine\\ 
\hline
I don't think the vaccine is necessary\\ 
\hline
I don't trust the companies producing the vaccines\\ 
\hline
I don't want my children to get the vaccine\\ 
\hline
 \end{tabular}
 \end{center}
 \caption{Intents covered by \systemname.}
\end{table}




\begin{table}[t]
\small
\begin{center}
\begin{tabular}{ |p{7cm}|  }
\hline
intent\\ 
\hline
I think the vaccine was not tested on my community\\ 
\hline
I'm not sure the vaccine is effective enough\\ 
\hline
I'm waiting to see how it affects others\\ 
\hline
COVID vaccines can be worse than the disease itself\\ 
\hline
 Long term side-effects were not researched enough\\ 
\hline
Are regular safety measures enough to stay healthy?\\ 
\hline
Should people that had COVID get the vaccine?\\ 
\hline
Side effects and adverse reactions worry me\\ 
\hline
The COVID vaccine is not safe\\ 
\hline
The vaccine should not be mandatory\\ 
\hline
Do vaccines work against the mutated strains of COVID-19?\\ 
\hline
They will put a chip/microchip to manipulate me\\ 
\hline
What can this chatbot do?\\ 
\hline
What is in the vaccine?\\ 
\hline
Which one of the vaccines should I take?\\ 
\hline
Will I test positive after getting the vaccine?\\ 
\hline
Can other vaccines protect me from COVID-19?\\ 
\hline
Do I qualify for the vaccine?\\ 
\hline
I don't trust vaccines if they're from China or Russia\\ 
\hline
Are the side effects worse for the second shot\\ 
\hline
Can I get a second dose even after a COVID exposure?\\ 
\hline
Can I get other vaccines at the same time?\\ 
\hline
Can I get the vaccine if I have allergies?\\ 
\hline
Can I get the vaccine if I have had allergic reactions to vaccines before?\\ 
\hline
Can I have the vaccine as a Catholic? \\ 
\hline
Can I have the vaccine if I'm allergic to penicillin?\\ 
\hline
Can I still get COVID even after being vaccinated?\\ 
\hline
Can you mix the vaccines?\\ 
\hline
COVID-19 vaccines cause brain inflammation\\ 
\hline
Do the COVID-19 vaccines cause Bell's palsy?\\ 
\hline
"Do the mRNA vaccines contain preservatives, like thimerosal?"\\ 
\hline
Do the vaccines work in obese people?\\ 
\hline
Do you have to be tested for COVID before you vaccinated?\\ 
\hline
Does the vaccine contain animal products?\\ 
\hline
Does the vaccine contain live COVID virus?\\ 
\hline
Does the vaccine impact pregnancy?\\ 
\hline
Does the vaccine work if I do not experience any side effects?\\ 
\hline
How can I stay safe until I'm vaccinated?\\ 
\hline
"How do I know I'm getting a legitimate, authorized vaccine?"\\ 
\hline
How do I report an adverse reaction or side-effect \\ 
\hline
How long do I have to wait between doses?\\ 
\hline
How many doses do I need?\\ 
\hline
How was the vaccine tested?\\ 
\hline
I am concerned about getting the vaccine because of my medications.\\ 
\hline
I don't want the v-safe app monitoring or tracking me\\ 
\hline
I don't want to share my personal information \\ 
\hline
Is breastfeeding safe with the vaccine\\ 
\hline
Is the Johnson \& Johnson vaccine less effective than the others?\\ 
\hline
 \end{tabular}
 \end{center}
 \caption{Intents covered by \systemname cont.}
\end{table}




\begin{table}[t]
\small
\begin{center}
\begin{tabular}{ |p{7cm}|  }
\hline
intent\\ 
\hline
Is the vaccine halal? \\ 
\hline
Is the vaccine Kosher?\\ 
\hline
Is there vaccine safety monitoring?\\ 
\hline
Other vaccines have caused long-term health problems\\ 
\hline
Should I get the COVID-19 vaccine if I am immunocompromised\\ 
\hline
Should I get the vaccine if I've tested positive for antibodies?\\ 
\hline
The vaccine includes fetal tissue or abortion by-products\\ 
\hline
The vaccine was rushed\\ 
\hline
Vaccine side effects are not getting reported\\ 
\hline
What does vaccine efficacy mean?\\ 
\hline
What if I still get infected even after receiving the vaccine?\\ 
\hline
What if I've been treated with convalescent plasma? \\ 
\hline
What if I've been treated with monoclonal antibodies?\\ 
\hline
What is mRNA?\\ 
\hline
What is the difference between mRNA and viral vector vaccines? \\ 
\hline
When can I go back to normal life? \\ 
\hline
Why are there different vaccines?\\ 
\hline
Why do I need the COVID vaccine if I don't get immunized for flu\\ 
\hline
Why do we need the vaccine if we can wait for herd immunity?\\ 
\hline
Why get vaccinated if I can still transmit the virus?\\ 
\hline
Will 1 dose of vaccine protect me?\\ 
\hline
Can I take a pain reliever when I get vaccinated?\\ 
\hline
Will the vaccine benefit me?\\ 
\hline
Will the vaccine make me sterile or infertile?\\ 
\hline
Can we change the vaccine quickly if the virus mutates?\\ 
\hline
Can I get COVID-19 from the vaccine?\\ 
\hline
I'm still experiencing COVID symptoms even after testing negative - should I still take the vaccine?\\ 
\hline
 Can children get the vaccine?\\ 
\hline
 Can we choose which vaccine we want?\\ 
\hline
 How long does the immunity from the vaccine last?\\ 
\hline
" The mortality rate of COVID-19 is low, why should I get the vaccine?"\\ 
\hline
 There are many reports of severe side effects or deaths from the vaccine\\ 
\hline
How can I get the vaccine?\\ 
\hline
I am worried about blood clots as a result of the vaccine\\ 
\hline
what is covid?\\ 
\hline
Who developed the vaccine?\\ 
\hline
Which vaccines are available?\\ 
\hline
What are the side effect of the vaccine?\\ 
\hline
Can I meet in groups after I'm vaccinated? \\ 
\hline
Is it safe to go to the gym indoors if I'm vaccinated? \\ 
\hline
How do I protect myself indoors? \\ 
\hline
What are the effects of long COVID?\\ 
\hline
Do you need a social security number to get a COVID-19 vaccine? \\ 
\hline
Do you need to be a U.S. citizen to get a COVID-19 vaccine? \\ 
\hline
Is it okay for me to travel internationally if I'm vaccinated? \\ 
\hline
 \end{tabular}
 \end{center}
 \caption{Intents covered by \systemname cont.}
\end{table}




\begin{table}[t]
\small
\begin{center}
\begin{tabular}{ |p{7cm}|  }
\hline
intent\\
\hline
Can my kids go back to school without a vaccine?\\ 
\hline
Will I need a booster shot? \\ 
\hline
"If I live with an immuno-compromised individual, do I still need to wear a mask outdoors if I'm vaccinated? "\\ 
\hline
Does the vaccine prevent transmission? \\ 
\hline
Why is AstraZeneca not approved in the USA?\\ 
\hline
Do I need to change my masking and social distancing practices depending on which COVID-19 vaccine I got? \\ 
\hline
Does the Pfizer vaccine cause myocarditis? \\ 
\hline
Does the Pfizer vaccine cause heart problems? \\ 
\hline
What can you tell me about COVID-19 vaccines?\\ 
\hline
Are there medical contraindications to the vaccines?\\ 
\hline
How many people died from COVID-19?\\ 
\hline
What about reports of abnormal periods due to the vaccine?\\ 
\hline
Do I need the vaccine?\\ 
\hline
Tell me about the vaccine\\ 
\hline
Is the Pfizer vaccine safe for young men?\\ 
\hline
Will vaccination lead to more dangerous variants?\\ 
\hline
Is it safe for my baby to get the vaccine?\\ 
\hline
Did a volunteer in the Oxford trial die?\\ 
\hline
Can I get COVID-19 twice?\\ 
\hline
Are some vaccines safer for younger children than others?\\ 
\hline
How long am I immune from COVID-19 if I had the virus?\\ 
\hline
Are women more likely to get worse side effects than men?\\ 
\hline
How do I convince my family and friends to get the COVID-19 vaccine?\\ 
\hline
Why are COVID-19 vaccination rates slowing in the U.S.?\\ 
\hline
I'm going to get vaccinated\\ 
\hline
Is getting vaccinated painful?\\ 
\hline
What do I do if I lose my COVID-19 vaccination card?\\ 
\hline
Can I get swollen lymph nodes from the vaccine?\\ 
\hline
Can my newborn become immune to COVID-19 if I'm vaccinated?\\ 
\hline
"COVID-19 is over, why should I get the vaccine?"\\ 
\hline
Did one woman die after getting the J\&J vaccine?\\ 
\hline
Do people become magnetic after getting vaccinated?\\ 
\hline
Does the vaccine contain eggs?\\ 
\hline
How is the COVID-19 vaccine different than others?\\ 
\hline
How soon after I've had COVID-19 can I get the vaccination?\\ 
\hline
Is it safe for my teen to get the vaccine?\\ 
\hline
Is this Pfizer vaccine equally effective in kids as it is in adults?\\ 
\hline
Were the COVID-19 vaccines tested on animals?\\ 
\hline
What are the side effects of the vaccine in children?\\ 
\hline
What is the delta variant?\\ 
\hline
What is the J\&J vaccine?\\ 
\hline
What is the Moderna vaccine?\\ 
\hline
What is the Pfizer vaccine?\\ 
\hline
Where are we required to wear masks now?\\ 
\hline
Who can get the Pfizer vaccine?\\ 
\hline
Who can I talk to about COVID-19 in person?\\ 
\hline
\end{tabular}
 \end{center}
 \caption{Intents covered by \systemname cont.}
\end{table}




\begin{table}[t]
\small
\begin{center}
\begin{tabular}{ |p{7cm}|  }
\hline
intent\\
\hline
Why should I trust you?\\ 
\hline
Will my child need my permission to get vaccinated?\\ 
\hline
Will the US reach herd immunity?\\ 
\hline
Will my child miss school when they get vaccinated?\\ 
\hline
Is the vaccine FDA approved?\\ 
\hline
Why do vaccinated people need to wear a mask indoors?\\ 
\hline
Do vaccinated people need to quarantine if exposed to COVID-19?\\ 
\hline
What is Ivermectin?\\ 
\hline
Does the Johnson and Johnson vaccine cause Rare Nerve Syndrome?\\ 
\hline
What is the difference between quarantine and isolation?\\ 
\hline
Does the COVID-19 vaccine cause autism?\\ 
\hline
Does the vaccine cause impotence?\\ 
\hline
Who is required to get vaccinated under the federal vaccine mandate?\\ 
\hline
Is the Delta variant more dangerous for kids?\\ 
\hline
Will there be a booster shot for J\&J and Moderna?\\ 
\hline
Is the booster the same as the original vaccine?\\ 
\hline
What are the side effects of booster shots?\\ 
\hline
What is the difference between the third shot and a booster shot?\\ 
\hline
How common are vaccine side effects?\\ 
\hline
Why do my kids need a vaccine if they're unlikely to get sick with COVID-19?\\ 
\hline
What happens if there is a COVID-19 case at my child's school?\\ 
\hline
Are booster shot side effects worse than those from the second shot?\\ 
\hline
Is the booster shot dangerous?\\ 
\hline
Can I get the vaccine if I have Multiple Sclerosis?\\ 
\hline
Do children receive the same dose of Pfizer as adults?\\ 
\hline
What is the Omicron variant?\\ 
\hline
How effective is the vaccine against the Omicron variant?\\
\hline
 \end{tabular}
 \end{center}
 \caption{Intents covered by \systemname cont.}
\end{table}








